The Role of Magnetic Helicity in the Structure and Heating of the Sun's Corona

Two of the most important features of the solar atmosphere are its hot, smooth coronal loops and the concentrations of magnetic shear, known as filament channels, that reside above photospheric polarity inversion lines (PILs). The shear observed in filament channels represents magnetic helicity, while the smoothness of the coronal loops indicates an apparent lack of magnetic helicity in the rest of the corona. At the same time, models that attempt to explain the high temperatures observed in these coronal loops require magnetic energy, in the form of twist, to be injected at the photosphere. In addition to magnetic energy, this twist also represents magnetic helicity. Unlike magnetic energy, magnetic helicity is conserved under reconnection, and is consequently expected to accumulate and be observed in the corona. However, filament channels, rather than the coronal loops, are the locations in the corona where magnetic helicity is observed, and it manifests itself in the form of shear, rather than twist. This naturally raises the question: if magnetic helicity needs to be injected to heat coronal loops, why is it only observed in filament channels, while coronal loops are observed to be laminar and smooth? This thesis addresses this question using a series of numerical simulations that demonstrate that magnetic helicity is transported throughout the solar corona by magnetic reconnection in such a way that it accumulates above PILs, forming filament channels, and leaving the rest of the corona generally smooth. In the process, it converts magnetic energy into heat, accounting for the large observed temperatures. This thesis presents a model for the formation of filament channels in the solar corona and the presence of smooth, hot coronal loops, and shows how the transport of magnetic helicity throughout the solar corona by magnetic reconnection is responsible for both of these phenomena.

==> glossary.tex <==
% this file is called up by thesis.tex
% content in this file will be fed into the main document

% Glossary entries are defined with the command \nomenclature{1}{2}
% 1 = Entry name, e.g. abbreviation; 2 = Explanation
% You can place all explanations in this separate file or declare them in the middle of the text. Either way they will be collected in the glossary.

% required to print nomenclature name to page header
%\markboth{\MakeUppercase{\nomname}}{\MakeUppercase{\nomname}}


% ----------------------- contents from here ------------------------

% chemicals
5\nomenclature{DAPI}{4',6-diamidino-2-phenylindole; a fluorescent stain that binds strongly to DNA and serves to marks the nucleus in fluorescence microscopy} 
\nomenclature{DEPC}{diethyl-pyro-carbonate; used to remove RNA-degrading enzymes (RNAases) from water and laboratory utensils}
\nomenclature{DMSO}{dimethyl sulfoxide; organic solvent, readily passes through skin, cryoprotectant in cell culture}
\nomenclature{EDTA}{Ethylene-diamine-tetraacetic acid; a chelating (two-pronged) molecule used to sequester most divalent (or trivalent) metal ions, such as calcium (Ca$^{2+}$) and magnesium (Mg$^{2+}$), copper (Cu$^{2+}$), or iron (Fe$^{2+}$ / Fe$^{3+}$)}

